Regret Analysis of Bandit Problems with Causal Background Knowledge

We study how to learn optimal interventions sequentially given causal information represented as a causal graph along with associated conditional distributions. Causal modeling is useful in real world problems like online advertisement where complex causal mechanisms underlie the relationship between interventions and outcomes. We propose two algorithms, causal upper confidence bound (C-UCB) and causal Thompson Sampling (C-TS), that enjoy improved cumulative regret bounds compared with algorithms that do not use causal information. We thus resolve an open problem posed by \cite{lattimore2016causal}. Further, we extend C-UCB and C-TS to the linear bandit setting and propose causal linear UCB (CL-UCB) and causal linear TS (CL-TS) algorithms. These algorithms enjoy a cumulative regret bound that only scales with the feature dimension. Our experiments show the benefit of using causal information. For example, we observe that even with a few hundreds of iterations, the regret of causal algorithms is less than that of standard algorithms by a factor of three. We also show that under certain causal structures, our algorithms scale better than the standard bandit algorithms as the number of interventions increases.

==> causal_linear.tex <==
Previous section demonstrates how we use causal knowledge to improve the multi-armed bandit algorithms. In our setting, the reward $Y$ directly depends on its $n$ parent nodes, then a natural extension is to consider the linear modeling case:
\begin{align}
	Y|_{\text{Pa}_Y=\mathbf{Z}} = f(\mathbf{Z})^T\theta + \epsilon,
\end{align}
where $f$ denotes the feature function applied on the parent nodes of $Y$, $\theta$ denotes the linear coefficient and $\epsilon$ is a zero mean, 1-subgaussian distributed random error.

We can write the expected reward mean for $\forall a\in\mathcal{A}$ as:
\begin{align}
	\mu_a &= \sum_{j=1}^{k^n}\mathbb{E}\left[Y|\text{Pa}_Y=\mathbf{Z}_j\right]P(\text{Pa}_Y=\mathbf{Z}_j|a)\\
	%&= \sum_{j=1}^{k^n}f(\mathbf{Z}_j)^T\theta P(\text{Pa}_Y=\mathbf{Z}_j|a)\\
	&= \langle \sum_{j=1}^{k^n}f(\mathbf{Z}_j)P(\text{Pa}_Y=\mathbf{Z}_j|a),\theta\rangle.
\end{align}
To this point, we demonstrate that linearly modeling the reward's parent nodes is just a special case of standard linear bandit problem, where the feature vector for $a\in\mathcal{A}$ is $m_a:=\sum_{j=1}^{k^n}f(\mathbf{Z}_j)P(\text{Pa}_Y=\mathbf{Z}_j|a)$. Thus, we easily extend C-UCB and C-TS to this particular linear bandit setting. 



\subsection{Causal Linear UCB (CL-UCB) \& Causal Linear TS (CL-TS)}
CL-UCB and CL-TS are straightforward linear UCB and linear TS algorithms. It is helpful in the sense that the regret dependence on $\sqrt{k^n}$ can be further reduced to the dimension of linear coefficient $\theta$ denoted by $d$. 

\begin{thm}[Regret Bound for CL-UCB \& CL-TS adapted from Chapter 19 in~\citet{lattimore2018bandit}] \label{thm:CL}
	Assume that $\left\|\theta\right\|_2 \leq 1$ and $\left\|f(\mathbf{Z})\right\|_2\leq 1$, the dimension of $\theta$ and $f(\mathbf{Z})$ are both $d$, then run CL-UCB with $\beta = 1+\sqrt{2\log\left(T\right)+d\log\left(1+\frac{T}{d}\right)}$ and CL-TS, the regret of CL-UCB and Bayesian regret of CL-TS can both be bounded by
	\begin{align}
	\mathbb{E}\left[R_{T_{CL-UCB}}\right], BR_{T_{CL-TS}} 
	%&\leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{T}{d}\right)}\\
	&= \tilde{O}\left(d\sqrt{T}\right).
	\end{align}
\end{thm}


